How to Cooperate Locally to Improve Global Privacy in Social Networks? On Amplification of Privacy Preserving Data Aggregation

In many systems privacy of users depends on the number of participants applying collectively some method to protect their security. Indeed, there are numerous already classic results about revealing aggregated data from a set of users. The conclusion is usually as follows: if you have enough friends to "aggregate" the private data, you can safely reveal your private information. Apart from data aggregation, it has been noticed that in a wider context privacy can be often reduced to being hidden in a crowd. Generally, the problems is how to create such crowd. This task may be not easy in some distributed systems, wherein gathering enough "individuals" is hard for practical reasons. Such example are social networks (or similar systems), where users have only a limited number of semi trusted contacts and their aim is to reveal some aggregated data in a privacy preserving manner. This may be particularly problematic in the presence of a strong adversary that can additionally corrupt some users. We show two methods that allow to significantly amplify privacy with only limited number of local operations and very moderate communication overhead. Except theoretical analysis we show experimental results on topologies of real-life social networks to demonstrate that our methods can significantly amplify privacy of chosen aggregation protocols even facing a massive attack of a powerful adversary. We believe however that our results can have much wider applications for improving security of systems based on locally trusted relations.

==> biblio.tex <==
\begin{thebibliography}{10}

\bibitem{AbdallaModel}
Abdalla, M., Fouque, P., Pointcheval, D.:
\newblock Password-based authenticated key exchange in the three-party setting.
\newblock In Vaudenay, S., ed.: Public Key Cryptography - {PKC} 2005. 
\newblock   Vol. 3386 of LNCS, Springer (2005)  65--84

\bibitem{Barker:2007:SRK:2206273}
Barker, E.B., Barker, W.C., Burr, W.E., Polk, W.T., Smid, M.E.:
\newblock Sp 800-57. recommendation for key management, part 1: General
  (revised).
\newblock Technical report, Gaithersburg, MD, United States (2007)

\bibitem{DBLP:journals/jce/BeckerRPB14}
Becker, G.T., Regazzoni, F., Paar, C., Burleson, W.P.:
\newblock Stealthy dopant-level hardware trojans: extended version.
\newblock J. Cryptographic Engineering \textbf{4}(1) (2014)  19--31

\bibitem{DBLP:conf/crypto/BellarePR14}
Bellare, M., Paterson, K.G., Rogaway, P.:
\newblock Security of symmetric encryption against mass surveillance.
\newblock In Garay, J.A., Gennaro, R., eds.: Advances in Cryptology - {CRYPTO}. 
\newblock Vol. 8616 of LNCS, Springer (2014)  1--19

\bibitem{DBLP:journals/iacr/BellarePR14}
Bellare, M., Paterson, K.G., Rogaway, P.:
\newblock Security of symmetric encryption against mass surveillance.
\newblock {IACR} Cryptology ePrint Archive \textbf{2014} (2014)  438

\bibitem{DBLP:conf/isw/BenderFK09}
Bender, J., Fischlin, M., K{\"u}gler, D.:
\newblock Security analysis of the pace key-agreement protocol.
\newblock In Samarati, P., Yung, M., Martinelli, F., Ardagna, C.A., eds.: ISC.
  Vol. 5735 of LNCS,  Springer (2009)  33--48

\bibitem{bsi-03110-p3}
{BSI}:
\newblock {Advanced Security Mechanisms for Machine Readable Travel Documents
  2.11}.
\newblock Technische Richtlinie TR-03110-3 (2013)

\bibitem{BSI-CC-PP-0064}
{Bundesamt f\"ur Sicherheit in der Informationstechnik}:
\newblock {Common Criteria Protection Profile for Inspection Systems (IS)},
  {BSI-CC-PP-0064}.
\newblock
  \url{https://www.commoncriteriaportal.org/files/ppfiles/pp0064b_pdf.pdf}
  (2010)

\bibitem{DBLP:conf/eurocrypt/CanettiK01}
Canetti, R., Krawczyk, H.:
\newblock Analysis of key-exchange protocols and their use for building secure
  channels.
\newblock In Pfitzmann, B., ed.: EUROCRYPT. 
Vol. 2045 of LNCS, Springer (2001)  453--474

\bibitem{eIDAS}
{European Parliament and the Council}:
\newblock Regulation ({EU}) no 910/2014 on electronic identification and trust
  services for electronic transactions in the internal market and repealing
  {Directive 1999/93/EC}.
\newblock
  \url{http://eur-lex.europa.eu/legal-content/EN/TXT/HTML/?uri=CELEX:32014R091%
0&from=EN},  (2014)

\bibitem{DBLP:conf/ispec/HanzlikKK13}
Hanzlik, L., Krzywiecki, L., Kuty{\l}owski, M.:
\newblock Simplified {PACE|AA} protocol.
\newblock In Deng, R.H., Feng, T., eds.: ISPEC. Vol. 7863 of LNCS, Springer (2013)  218--232

\bibitem{PACEv2}
{ISO/IEC JTC1 SC17 WG3/TF5 for the International Civil Aviation Organization}:
\newblock Supplemental access control for machine readable travel documents.
\newblock Technical Report (2011) version 1.02, March 08.

\bibitem{SPEKE}
Jablon, D.P.:
\newblock Extended password key exchange protocols immune to dictionary
  attacks.
\newblock In: WETICE, IEEE Computer Society (1997)  248--255

\bibitem{ais20ais31}
Killmann, W., Schindler, W.:
\newblock A proposal for functionality classes for random number generators.
\newblock
  \url{https://www.bsi.bund.de/SharedDocs/Downloads/DE/BSI/Zertifizierung/Inte%
rpretationen/AIS_20_Functionality_classes_for_random_number_generators_e.pdf}
  (2011)

\bibitem{DBLP:journals/iacr/LaMacchiaLM06}
LaMacchia, B.A., Lauter, K., Mityagin, A.:
\newblock Stronger security of authenticated key exchange.
\newblock IACR Cryptology ePrint Archive \textbf{2006} (2006) ~73

\bibitem{DBLP:books/daglib/0020579}
Young, A.L., Yung, M.:
\newblock Malicious cryptography - exposing cryptovirology.
\newblock Wiley (2004)

\end{thebibliography}

